Chain-of-Action: Trajectory Autoregressive Modeling for Robotic Manipulation

We present Chain-of-Action (CoA), a novel visuo-motor policy paradigm built upon Trajectory Autoregressive Modeling. Unlike conventional approaches that predict next step action(s) forward, CoA generates an entire trajectory by explicit backward reasoning with task-specific goals through an action-level Chain-of-Thought (CoT) process. This process is unified within a single autoregressive structure: (1) the first token corresponds to a stable keyframe action that encodes the task-specific goals; and (2) subsequent action tokens are generated autoregressively, conditioned on the initial keyframe and previously predicted actions. This backward action reasoning enforces a global-to-local structure, allowing each local action to be tightly constrained by the final goal. To further realize the action reasoning structure, CoA incorporates four complementary designs: continuous action token representation; dynamic stopping for variable-length trajectory generation; reverse temporal ensemble; and multi-token prediction to balance action chunk modeling with global structure. As a result, CoA gives strong spatial generalization capabilities while preserving the flexibility and simplicity of a visuo-motor policy. Empirically, we observe CoA achieves the state-of-the-art performance across 60 RLBench tasks and 8 real-world manipulation tasks.

==> sec/0.abs.tex <==
% \begin{figure}[ht]
% \vspace{-16pt}
% \begin{center}
% 	\includegraphics[width=0.97\linewidth]{fig/abs.jpg}
% \end{center}
% \vspace{-7pt}
% \caption{\small
% \textbf{Generated samples from Visual AutoRegressive (VAR) transformers trained on ImageNet}.
% We show 512$\times$512 samples (top), 256$\times$256 samples (middle), and zero-shot image editing results (bottom).
% }
% \vspace{-2pt}
% \label{fig:abs}
% \end{figure}

\begin{abstract}
\vspace{-4pt}

% LNCS guidelines indicate it should be at least 70 and at most 150 words.
% Please include keywords as in the example below. 
% This is required for papers in LNCS proceedings.


% Robotic manipulation demands both reactivity and precision. Contemporary visuo‑motor approaches—particularly action‑chunking paradigms—learn closed‑loop policies that map observations directly to short sequences of actions. While these models enable real‑time adaptation, they frequently suffer from compounding errors as early inaccuracies propagate through execution. Hierarchical methods, by contrast, predict goal‑conditioned keyframe poses and employ motion planners to generate full trajectories, thereby ensuring global consistency. However, such approaches operate in an open‑loop fashion and lack the environment‑awareness necessary to adjust during execution.This motivates the question: \emph{can we bring the global intent-driven structure of hierarchical models into the reactive framework of visuo-motor control}? 
% We propose Trajectory Autoregressive Modeling, a new visuo-motor paradigm that reformulates action prediction as a reverse trajectory generation process---from a goal-related pose progressively back to the current gripper state. Our method, Chain-of-Action (CoA), explicitly models the trajectory as a chain of causally linked poses. This chain-structured reasoning ensures global consistency throughout the trajectory, aligning each local decision with the task objective and enabling goal-aware, closed-loop control.
% Evaluated on 50 tasks from the RLBench benchmark, CoA consistently outperforms strong visuo-motor baselines—including ACT and Diffusion Policy—under the same architecture with minimal modifications. Beyond overall accuracy, CoA demonstrates stronger spatial generalization, achieving superior interpolation and extrapolation performance. These results highlight reverse trajectory modeling as a promising direction for building robust and generalizable manipulation policies.

% Robotic manipulation today is dominated by reactive visuo‑motor policies—often implemented via action‑chunk prediction—that adapt in closed‑loop yet suffer from compounding errors as early inaccuracies reverberate through execution. Hierarchical methods, by predicting goal‑conditioned keyframe poses and invoking motion planners, guarantee global consistency but operate open‑loop and rely on heavy 3D sensing.  In this work, we ask: \emph{Can we endow a reactive visuo‑motor model with global intent, without relinquishing closed‑loop adaptability?}  We introduce \textbf{Chain‑of‑Action (CoA)}, a \emph{Trajectory Autoregressive Modeling} paradigm that generates a full trajectory in reverse: starting from the goal pose and stepping causally back to the current gripper state.  CoA weaves global task structure into each local decision, mitigating compounding errors and preserving closed‑loop reactivity at modest computational cost.  On 50 RLBench tasks, CoA—built on the same visuo‑motor backbone with only minor modifications—significantly outperforms leading chunk‑based baselines (e.g.\,ACT, Diffusion Policy), achieving superior accuracy and spatial generalization.  Our results demonstrate that reverse trajectory modeling can reconcile precision‑wise the strengths of hierarchical planning with the adaptability of closed‑loop control, pointing the way toward a new generation of visuo‑motor action models.

% Existing visuo-motor policies often struggle with poor generalization, even when trained on substantial amounts of data, seemingly constrained by an inherent limitation. We argue that this limitation arises fundamentally from their lack of explicit modeling of task-level intent, make train and test goal not aligned. 
We present \textbf{Chain-of-Action (CoA)}, a novel visuo-motor policy paradigm built upon \emph{Trajectory Autoregressive Modeling}. Unlike conventional approaches that predict next step action(s) \textit{forward}, CoA generates an entire trajectory by explicit \emph{backward} reasoning with task-specific goals through an action-level Chain-of-Thought (CoT) process. This process is unified within a single autoregressive structure: (1) the first token corresponds to a stable keyframe action that encodes the task-specific goals;  and (2) subsequent action tokens are generated autoregressively, conditioned on the initial keyframe and previously predicted actions.
This backward action reasoning enforces a global-to-local structure, allowing each local action to be tightly constrained by the final goal. To further realize the action reasoning structure, CoA incorporates four complementary designs: continuous action token representation; dynamic stopping for variable-length trajectory generation; reverse temporal ensemble; and multi-token prediction to balance action chunk modeling  with global structure. As a result, CoA gives strong spatial generalization capabilities while preserving the flexibility and simplicity of a visuo-motor policy. Empirically, we observe CoA achieves the state-of-the-art performance across 60 RLBench tasks and 8 real-world manipulation tasks.\footnote{Code will be open-sourced upon publication.}

% \textcolor{red}{This paper presents Chain-of-Action (CoA), a novel visuo-motor policy paradigm grounded in trajectory autoregressive modeling. Rather than predicting the next action in a forward manner, CoA begins by forecasting a task-specific keyframe action that encapsulates the ultimate goal. It then autoregressively generates each preceding action token in reverse, reasoning backward from that keyframe to the current state. This backward “chain-of-thought” binds every local decision tightly to the global objective, all within a single Transformer-based policy that remains end-to-end and easy to deploy.
% To realize this autoregressive backward reasoning, CoA weaves together four complementary designs. By representing actions as continuous tokens, it achieves high-resolution control; a dynamic stopping criterion automatically halts the rollout once it reaches the current state; reverse temporal ensembling merges multiple backward trajectories to reduce inference variance; and multi-token prediction balances the need for modeling fine-grained local dependencies with global consistency. Thanks to these innovations, CoA retains the simplicity of standard visuo-motor policies while delivering markedly stronger spatial generalization. Empirically, it outperforms leading baselines by 16–23\% on 60 RLBench tasks and yields a 33\% relative boost in success on eight real-robot manipulation scenarios, demonstrating the power and generality of backward, autoregressive action reasoning for long-horizon robotic manipulation.}


% derives action(s) causally from a goal pose gradually \textit{backward} to the current gripper state.

% This incorporates two essential innovations: (1) explicit definition of a stable, invariant task-level intent via the goal pose, and
% (2) an autoregressive modeling of the action chain that constrains each generated action by this intent. 
% % (2) an autoregressive modeling that step-by-step propagates task intent from the goal along the action chain to ultimately determine the current action to be executed.
% As a result, each local decision (derived action) robustly aligns with the stable task-level intent (goal pose), significantly improve the generalizaiton ability. Experiments conducted on 60 RLBench tasks demonstrate that CoA, implemented with minimal modifications to the ACT model, significantly outperforms state-of-the-art baselines (ACT and Diffusion Policy).


% Robotic manipulation today is dominated by reactive visuo‑motor policies—often implemented via action‑chunk prediction—that adapt in closed‑loop yet suffer from compounding errors as early inaccuracies reverberate through execution. Hierarchical methods, by predicting goal‑conditioned keyframe poses and invoking motion planners, guarantee global consistency but operate open‑loop and rely on heavy 3D sensing. In this work, we ask: \emph{Can we endow a reactive visuo‑motor model with global intent, without relinquishing closed‑loop adaptability?} We introduce \textbf{Chain‑of‑Action (CoA)}, a \emph{Trajectory Autoregressive Modeling} paradigm that generates a full trajectory in reverse: starting from the goal pose and stepping causally back to the current gripper state. CoA weaves global task structure into each local decision, mitigating compounding errors and preserving closed‑loop reactivity with minimal adaptation effort—requiring no extra annotations and only slight modifications to existing visuo‑motor policies. On 50 RLBench tasks, CoA—built on ACT with only minor changes—significantly outperforms leading baselines (e.g.\,ACT, Diffusion Policy), achieving superior accuracy and spatial generalization. Our results demonstrate that reverse trajectory modeling can reconcile precision‑wise the strengths of hierarchical planning with the adaptability of closed‑loop control, pointing the way toward a new generation of visuo‑motor action models.



\end{abstract}

% Comparison between conventional vision-action modeling paradigms and our proposed Chain-of-Action framework.}
% (a) \textit{Action chunk}-based methods: directly predict fixed-length action segments (chunks), often without explicit trajectory structure;
% (b) \textit{Hierarchical}-based methods: typically take RGB-D inputs to predict a next-best pose, then invoke a motion planner to compute the full trajectory;
% (c) \textit{Chain-of-Action} (ours): the entire trajectory is autoregressively generated from the goal pose back to the current gripper pose, in a continuous action embedding space, capturing long-horizon dependencies.

% \begin{figure}[ht]
% \centering
% \includegraphics[width=0.48\linewidth]{fig/teaser.pdf}
% \vspace{-6pt}
% \caption{\small
% \textbf{Comparison of (a) vanilla visuo-motor policy and (b) our Chain-of-Action.}
% }
% \vspace{-8pt}
% \label{fig:teaser}
% \end{figure}



==> sec/3.1.preliminary.tex <==
% Autoregressive modeling is originally designed for sequential data like language or flatten visual tokens. The key insight of it is to capture the underlying temporal dependencies by factorizing the data likelihood into a product of conditional probabilities. For a token sequence $x = (x_1, x_2, \dots, x_T)$, this is expressed as:

\vspace{-3pt}
\subsection{action chunk modeling} \label{sec:ar}
\vspace{-2pt}

\firstpara{Formulation.}

\para{Action chunk}

\para{Temporal ensemble}

\subsection{next best pose modeling} \label{sec:ar}
\vspace{-2pt}

\firstpara{Formulation.}


\para{motion planer}


